EdgeViTs: Competing Light-weight CNNs on Mobile Devices with Vision Transformers

Self-attention based models such as vision transformers (ViTs) have emerged as a very competitive architecture alternative to convolutional neural networks (CNNs) in computer vision. Despite increasingly stronger variants with ever-higher recognition accuracies, due to the quadratic complexity of self-attention, existing ViTs are typically demanding in computation and model size. Although several successful design choices (e.g., the convolutions and hierarchical multi-stage structure) of prior CNNs have been reintroduced into recent ViTs, they are still not sufficient to meet the limited resource requirements of mobile devices. This motivates a very recent attempt to develop light ViTs based on the state-of-the-art MobileNet-v2, but still leaves a performance gap behind. In this work, pushing further along this under-studied direction we introduce EdgeViTs, a new family of light-weight ViTs that, for the first time, enable attention-based vision models to compete with the best light-weight CNNs in the tradeoff between accuracy and on-device efficiency. This is realized by introducing a highly cost-effective local-global-local (LGL) information exchange bottleneck based on optimal integration of self-attention and convolutions. For device-dedicated evaluation, rather than relying on inaccurate proxies like the number of FLOPs or parameters, we adopt a practical approach of focusing directly on on-device latency and, for the first time, energy efficiency. Specifically, we show that our models are Pareto-optimal when both accuracy-latency and accuracy-energy trade-offs are considered, achieving strict dominance over other ViTs in almost all cases and competing with the most efficient CNNs. Code is available at https://github.com/saic-fi/edgevit.

==> code/pseudo_code.tex <==
\begin{lstlisting}[language=python]
class LocalAgg():
    def __init__(self, dim):
        self.conv1 = Conv2d(dim, dim, 1)
        self.conv2 = Conv2d(im, dim, 3, padding=1, groups=dim)
        self.conv3 = Conv2d(dim, dim, 1)
        self.norm1 = BatchNorm2d(dim)
        self.norm2 = BatchNorm2d(dim)
        
    def forward(self, x):
        """
        [B, C, H, W] = x.shape
        """
        x = self.conv1(self.norm1(x))
        x = self.conv2(x)
        x = self.conv3(self.norm2(x))
        return x

class GlobalSparseAttn():
    def __init__(self, dim, sample_rate, scale):
        self.scale = scale
        self.qkv = Linear(dim, dim * 3)
        self.sampler = AvgPool2d(1, stride=sample_rate)
        kernel_size=sr_ratio
        self.LocalProp = ConvTranspose2d(dim, dim, kernel_size, stride=sample_rate, groups=dim)
        self.norm = LayerNorm(dim)
        self.proj = Linear(dim, dim)
        
    def forward(self, x):
        """
        [B, C, H, W] = x.shape
        """
        x = self.sampler(x)
        q, k, v = self.qkv(x)

        attn = q @ k * self.scale
        attn = attn.softmax(dim=-1)
        x = attn @ v
        
        x = self.LocalProp(x)
        x = self.proj(self.norm(x))
        return x

class DownSampleLayer():
    def __init__(self, dim_in, dim_out, downsample_rate):
        self.downsample = Conv2d(dim_in, dim_out, kernel_size=downsample_rate, stride=downsample_rate)
        self.norm = LayerNorm(dim_out)

    def forward(self, x):
        x = self.downsample(x)
        x = self.norm(x)
        return x
        
class PatchEmbed():
    def __init__(self, dim):
        self.embed = Conv2d(dim, dim, 3, padding=1, groups=dim)

    def forward(self, x):
        return x + self.embed(x)
        
class FFN():
    def __init__(self, dim):
        self.fc1 = nn.Linear(dim, dim*4)
        self.fc2 = nn.Linear(dim*4, dim)

    def forward(self, x):
        x = self.fc1(x)
        x = GELU(x)
        x = self.fc2(x)
        return x

\end{lstlisting}

==> tables/cls_table_main.tex <==
\begin{tabular}{@{}l|x{45}|x{45}|x{45}@{}}
\toprule
 Model & \#Params & FLOPs & Top-1 \\
%\shline
\toprule
 {MobileNet-v2} \cite{mobilenetv2_cvpr18} & \bf 3.4M & 0.3G & 72.0\\
 {MobileNet-v3 1.0} \cite{mobilenetv3_iccv19} & 5.4M & \bf 0.2G & 75.2\\
 {MobileNet-v3 0.75} \cite{mobilenetv3_iccv19} & 4.0M & 0.16G & 73.3\\

 {EfficientNet-B0} \cite{tan2019efficientnet} & 5.3M & 0.4G & \bf 77.1\\
 %\hline
 \midrule
  {MobileViT-XXS*} \cite{mehta2021mobilevit}& \bf 1.3M & \bf 0.4G & 69.0 \\
  {PVT-v2-B0} \cite{wang2021pvtv2} & 3.4M & 0.6G & 70.5\\
  {Uniformer-Tiny*}\cite{uniformer_iclr22} & 3.9M & 0.6G & 74.1\\
  {Twins-Tiny*}\cite{chu2021twins} & 4.1M & 0.6G & 71.2 \\
%   {ConT-Tiny} \cite{xiao2021early}& 5.8M & 0.8G & 74.9 \\
  {\bf \netname-XXS} & 4.1M & 0.6G & \bf 74.4 \\
   \midrule
 {MobileViT-XS*} \cite{mehta2021mobilevit}& \bf 2.4M & 1.1G & 74.7 \\
 {T2T-ViT-7} \cite{yuan2021tokens}& 4.3M & 1.1G & 71.7 \\
 {Deit-Tiny} \cite{touvron2021training}& 5.7M & 1.3G & 72.2 \\
 {TNT-Tiny} \cite{han2021transformer}& 6.1M & 1.4G & 73.9 \\
 {ConT-Small} \cite{xiao2021early}& 10.1M & 1.5G & 76.5 \\
  {\bf \netname-XS} & 6.7M & \bf 1.1G & \bf 77.5 \\
%\hline
%\midrule
%\hline
\midrule
 {T2T-ViT-12} \cite{yuan2021tokens}& 6.9M & 1.9G & 76.5 \\
 {MobileViT-S*} \cite{mehta2021mobilevit}& \bf 5.6M & 2.0G & 78.3 \\
 {PVT-v2-B1} \cite{wang2021pvtv2} & 14M & 2.1G & 78.7\\
 {\bf \netname-S} & 11.1M & \bf 1.9G & \bf 81.0 \\
%\hline
\bottomrule
\end{tabular}

==> tables/cls_table_speed.tex <==
\tablestyle{4.8pt}
{1.1}\begin{tabular}{@{}l|x{37}|x{45}|x{45}|x{45}@{}}
\toprule
 Model & \#Params & FLOPs & CPU & Acc Top-1 \\
\toprule
 {MobileNet-v2}\cite{mobilenetv2_cvpr18} & \bf 3.4M & 0.3G & 33.3ms & 72.0 \\
 {MobileNet-v3 0.75}\cite{mobilenetv3_iccv19} & 4.0M & \bf 0.16G & \bf{23.0ms} & 73.3 \\
 {EfficientNet-B0}\cite{tan2019efficientnet} & 5.3M & 0.4G & 52.1ms & \bf 77.1 \\
  \midrule
 {MobileViT-XXS} \cite{mehta2021mobilevit}& \bf 1.3M & \bf 0.4G & 69.5ms & 69.0\\
 {PVT-v2-B0}\cite{wang2021pvtv2} & 3.4M & 0.6G & \bf 26.0ms & 70.5\\
 {Uniformer-Tiny*}\cite{uniformer_iclr22} & 3.9M & 0.6G & 40.5ms & 74.1\\
 {Twins-SVT-Tiny*}\cite{chu2021twins} & 4.1M & 0.6G & 36.9ms & 71.2\\
 {\bf \netname-XXS} & 4.1M & 0.6G & 32.8ms & \bf 74.4 \\
 \midrule
 {T2T-ViT-7} \cite{t2tvit}& 4.3M & 1.1G & 48.8ms &71.7 \\
 {MobileViT-XS} \cite{mehta2021mobilevit}& \bf 2.4M & 1.1G & 150.1ms & 74.7\\
 {DeiT-Tiny} \cite{deit2021}& 5.7M & 1.3G &  \bf 46.2ms & 72.2\\
 {TNT-Tiny} \cite{han2021transformer}& 6.1M & 1.4G & 86.4ms &73.9 \\
 {T2T-ViT-10} \cite{t2tvit}& 5.9M & 1.5G & 60.7ms &75.2 \\
 {\bf \netname-XS} & 6.7M & \bf 1.1G & 54.1ms & \bf 77.5 \\
 \midrule
 {T2T-ViT-12} \cite{t2tvit}& 6.9M & 1.9G & \bf 69.9ms &76.5 \\
 {PVT-v2-B1}\cite{wang2021pvtv2} & 14M & 2.1G & 75.4ms & 78.7\\
%  {Uniformer-Tiny*}\cite{uniformer_iclr22} & 3.9M & 0.6G & 74.1 & 40.52ms\\
%  {Twins-Tiny*}\cite{chu2021twins} & 4.1M & 0.6G & 71.2 & 36.9ms\\
%  {T2T-ViT-7} \cite{yuan2021tokens}& 4.3M & 1.1G & 48.8ms &71.7 \\
%  {TNT-Tiny} \cite{han2021transformer}& 6.1M & 1.4G & 86.4ms &73.9 \\
%  {T2T-ViT-10} \cite{yuan2021tokens}& 5.9M & 1.5G & 69.9ms &75.2 \\
%  {T2T-ViT-12} \cite{yuan2021tokens}& 6.9M & 1.9G & 69.9ms &76.5 \\
%  {MobileViT-XXS} \cite{mehta2021mobilevit}& 1.3M & 0.4G & 69.0 & 69.5ms \\
%  {MobileViT-XS} \cite{mehta2021mobilevit}& 2.4M & 1.1G & 74.7 & 150.1ms\\
 {MobileViT-S} \cite{mehta2021mobilevit}& \bf 5.6M & 2.0G & 221.3ms & 78.3\\
%   \midrule
%  {\bf \netname-XXS} & 4.1M & 0.6G & 74.4 & 32.8ms\\
%  {\bf \netname-XS} & 6.7M & 1.1G & 77.5 & 54.1ms \\
 {\bf \netname-S} & 11.1M & \bf 1.9G & 85.3ms & \bf{81.0} \\
 \hline
 
\end{tabular}

%   {ConT-Small} \cite{xiao2021early}& 10.1M & 1.5G & - &76.5 \\


==> tables/det_table_maskrcnn.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{l|c|ccc|ccc}
\toprule
%\renewcommand{\arraystretch}{0.1}
\multirow{2}{*}{Backbone} &\multicolumn{7}{c}{Mask R-CNN 1$\times$}\\ %&\multicolumn{7}{c}{Mask R-CNN 1$\times$} \\
\cmidrule{2-8}  %\cline{2-8} 
&  \#Par (M) &AP$^{\rm b}$ &AP$_{50}^{\rm b}$ &AP$_{75}^{\rm b}$  &AP$^{\rm m}$ &AP$_{50}^{\rm m}$ &AP$_{75}^{\rm m}$\\
\midrule
%\shline
PVTv2-B0~\cite{wang2021pvtv2} &\textbf{23.5} & 38.2 & 60.5 & 40.7 & 36.2 & 57.8 & 38.6  \\
\bf\netname-XXS & 23.8 & \textbf{39.9} & \textbf{62.0} & \textbf{43.1} & \textbf{36.9} & \textbf{59.0} & \textbf{39.4}  \\
\midrule
%\hline
\bf \netname-XS & 26.5 & 41.4 & 63.7 & 45.0 & 38.3 & 60.9 & 41.3  \\
\midrule
%\hline
ResNet18~\cite{he2016deep} &\textbf{31.2} & 34.0 & 54.0 & 36.7 & 31.2 & 51.0 & 32.7\\
PVTv1-Tiny~\cite{pvt} &32.9 & {36.7} & {59.2} & {39.3} & {35.1} & {56.7} & {37.3} \\
PVTv2-B1~\cite{wang2021pvtv2} &33.7 & 41.8 & 64.3 & 45.9 & 38.8 & 61.2 & 41.6 \\
\bf \netname-S & 32.8 & \textbf{44.8} & \textbf{67.4} & \textbf{48.9} & \textbf{41.0} & \textbf{64.2} & \textbf{43.8}  \\
\bottomrule
\end{tabular}

==> tables/det_table_retina_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{l|c|ccc|ccc}
\toprule
%\renewcommand{\arraystretch}{0.1}
\multirow{2}{*}{Backbone} &\multicolumn{7}{c}{RetinaNet 1$\times$}\\ %&\multicolumn{7}{c}{Mask R-CNN 1$\times$} \\
\cmidrule{2-8}  %\cline{2-8} 
& \#Par (M) & AP & AP$_{50}$ & AP$_{75}$ & AP$_S$ & AP$_M$ & AP$_L$ \\
% \midrule
\toprule %\shline
PVTv2-B0~\cite{wang2021pvtv2} & \textbf{13.0} & 37.2 & 57.2 & 39.5 & \textbf{23.1} & 40.4 & 49.7\\  
%\midrule%
\bf \netname-XXS  & 13.1 & \textbf{38.7} & \textbf{59.0} & \textbf{41.0} & 22.4 & \textbf{42.0} & \textbf{51.6}  \\
\midrule %\hline
\bf \netname-XS  & 16.3 & 40.6 & 61.3 & 43.3 & 25.2 & 43.9 & 54.6  \\
\midrule %\hline
ResNet18~\cite{he2016deep} &\textbf{21.3} & 31.8 & 49.6 & 33.6 & 16.3 & 34.3 & 43.2 \\ 
PVTv1-Tiny~\cite{pvt} &23.0& {36.7}& {56.9}& {38.9}& {22.6}& {38.8} &{50.0}\\
PVTv2-B1~\cite{wang2021pvtv2} &23.8 & 41.2 & 61.9 & 43.9 & 25.4 & 44.5 & 54.3\\
\bf \netname-S  & 22.6 & \textbf{43.4} & \textbf{64.9} & \textbf{46.5} & \textbf{26.9} & \textbf{47.5} & \textbf{58.1}  \\
\bottomrule
\end{tabular}
